RayZer: A Self-supervised Large View Synthesis Model

We present RayZer, a self-supervised multi-view 3D Vision model trained without any 3D supervision, i.e., camera poses and scene geometry, while exhibiting emerging 3D awareness. Concretely, RayZer takes unposed and uncalibrated images as input, recovers camera parameters, reconstructs a scene representation, and synthesizes novel views. During training, RayZer relies solely on its self-predicted camera poses to render target views, eliminating the need for any ground-truth camera annotations and allowing RayZer to be trained with 2D image supervision. The emerging 3D awareness of RayZer is attributed to two key factors. First, we design a self-supervised framework, which achieves 3D-aware auto-encoding of input images by disentangling camera and scene representations. Second, we design a transformer-based model in which the only 3D prior is the ray structure, connecting camera, pixel, and scene simultaneously. RayZer demonstrates comparable or even superior novel view synthesis performance than ``oracle'' methods that rely on pose annotations in both training and testing. Project: https://hwjiang1510.github.io/RayZer/

==> sections/legacy_01_introduction_0.tex <==
\section{Introduction}
The scaling law~\cite{} drives the progress in large foundation models, particularly in language (LLMs)~\cite{} and vision-language models (VLMs)~\cite{}. Yet, scaling 3D Vision models, which provide spatial intelligence, has lagged behind.

To scale up 3D Vision models, we draw insights from a more scalable modality--video generation models. Even though video generation models are not trained with any explicit knowledge of 3D, their 3D awareness emerge by looking at a large amount lot of videos~\cite{}. 
This success hinges on two key factors. First, these models, primarily based on DiT~\cite{}, incorporate \textit{minimal 3D inductive bias}, enabling greater flexibility and scalability~\cite{}. More importantly, they perform \textit{self-supervised learning} on unlabeled videos, unlocking the potential of training with mega-scale video data.

In contrast, current 3D Vision models is on the other extreme. They focus on embedding more 3D inductive biases at the architectural or representational level. At the same time, they relies heavily on fully supervised learning, using ground-truth camera poses for rendering or directly using 3D geometry supervision. These two constraints systematically limit scalability, both by restricting model capability and requiring precise yet costly supervision.


These observations raise a fundamental question: Is the scalability of 3D vision models inherently constrained by the use of 3D priors? In this paper, we investigate this hypothesis by introducing \textbf{\modelname{}}, a large-scale 3D vision model designed with \textit{least 3D inductive bias} -- \textbf{no explicit 3D representations}, \textbf{no 3D-informed architectures}, and, critically, \textbf{no 3D supervision for training}. As shown in Fig.~\ref{}, \modelname{} learns in a fully \textit{self-supervised} manner from unlabeled video frames, demonstrating \textbf{emerging 3D awareness}. It takes unposed and uncalibrated continuous video frames as input and accomplishes a wide range of 3D vision tasks, i.e. camera pose estimation, camera calibration, latent scene reconstruction, and novel view synthesis.

The power of \modelname{} stems from two key aspects. First, the core of \modelname{} model architecture is employing a ray-based representation to bridge 2D pixels and 3D space. Unlike previous approaches that impose hand-crafted inductive biases to model ray physics~\cite{}, we argue that the essence of rays lies in their pixel-aligned \textbf{ray structure}--how they propagate through space, accumulate to form pixel values, and establish cross-view correspondences should be fully learnable. Thus, we build on a full transformer-based model with a latent scene representation, injecting nearly zero 3D inductive bias.

% The power of \modelname{} comes from two aspects. First, the core of \modelname{} model is using ray-based representations to bridge 2D pixels and 3D space. Departing from previous works leveraging hand-crafted inductive bias for modeling the physical perspectives of rays, we argue that the essence of rays is the pixel-aligned \textbf{ray structure} -- how the rays are transmitted in space, how they accumulate to get 2D pixel values, and how they reveals cross-view correspondences can all be learned. Motivated by this understanding, we build a full transformer-based model with latent scene representation.


Second, this ray-based representation also facilitates self-supervised learning. While jointly predicting structure and motion is a classic chicken-and-egg problem that often leads to trivial solutions, the ray-based formulation turns out to be a strong regularization for meaningful learning. Specifically, \modelname{} first estimates camera parameters, including intrinsics and per-view camera poses. Then \modelname{} turns the predicted camera parameters as Plücker rays~\cite{} to condition latent scene reconstruction. Finally, it uses these Plücker rays to query the latent scene representation and render input images. This pipeline enables \modelname{} to learn 3D-aware representations purely from image supervision, achieving auto-encoding.

\modelname{} is trained xx


==> sections/legacy_01_introduction_1.tex <==
\section{Introduction}
\label{sec: intro}


% first paragraph got deleted..

To pursue scaling, in this paper, we explore how far we can push a multi-view 3D Vision model with \textbf{using the least 3D priors}. This exploration incorporates two keypoints, motivated by \textit{what 3D Vision models are missing} compared with other modalities. The most crucial aspect is \textbf{self-supervised learning}, i.e., using \textit{zero 3D supervision}, which is the fundamental reason for the observed scaling effects. By \textit{designing a effective self-supervised task}, we aim to break free from the bottleneck of expensive 3D data collection and annotation. While prior works have explored self-supervised learning~\cite{}, we demonstrate how it interacts synergistically with our second key aspect: \textbf{a pure transformer-based model} \textit{with minimal 3D inductive bias}. The removal of domain-specific knowledge, as seen in large-scale models across different fields~\cite{}, enables more flexible and scalable learning. Instead of incorporating 3D inductive bias, i.e., handcrafted 3D representations, rendering equations, network architectures, and learning regularization, we leverage the transformer’s capacity to learn generalizable patterns. Combining these two aspects, we aim at unlocking a more scalable path for 3D multi-view Vision models.


Based on \textit{the least 3D priors}, we design \textbf{\modelname{}}, a large-scale 3D Vision model showing \textbf{emerging 3D awareness}. \modelname{} focuses on multi-view 3D vision tasks. As shown in Fig.~\ref{}, \modelname{} learns in a fully \textit{self-supervised} manner from unlabeled multi-view images. \modelname{} focuses on multi-view 3D vision tasks. It takes \textit{unposed and uncalibrated images} as input and perform a wide range of classical 3D vision tasks, i.e., camera calibration and pose estimation, ``3D'' reconstruction, and novel view synthesis.


The least ``3D'' prior of \modelname{} is \textbf{adopting the concept of rays}, as rays can be the least physical knowledge to bridge 2D pixels (camera) and 3D space~\cite{}. Unlike previous approaches that impose hand-crafted inductive biases to model ray physics~\cite{}, we show that the essence of rays lies in their pixel-aligned \textbf{ray structure}--how they propagate through space, accumulate to form pixel values, and establish cross-view correlations can all be learned. 

This ray-structure prior facilitates self-supervised learning. While jointly predicting structure and motion is a classic chicken-and-egg problem that often leads to \textit{trivial solutions}~\cite{}, the ray-based formulation turns out to be a strong prior for meaningful learning. This is achieved, in our understanding, by letting camera and scene representations to \textbf{regularize each other} to pursue the global minima. Specifically, \modelname{} first estimates camera parameters, including intrinsics and per-view camera poses. Then \modelname{} turns the predicted camera parameters as Plücker rays~\cite{} to condition latent scene reconstruction. Finally, it uses these Plücker rays to query the latent scene representation and render input images. This pipeline enables \modelname{} to learn 3D-aware representations purely from image supervision, achieving 3D-aware auto-encoding of input images.

%Conceptually, \modelname{} and video generation models can be the two sides of the same coin -- video generation models are also built with transformer-based DiT~\cite{}, learning from unlabeled videos, and showing emerging 3D awareness~\cite{}. However, we demonstrate that with our least ``3D'' prior of using the ray structure, we can achieve unsupervised control of rendering viewpoint. In contrast, video generation models need to learn it during post-training with in a fully supervised manner. %The philosophical contribution of \modelname{} may unify 3D Vision and video generation for building a world model.


\modelname{} is trained xx


==> sections/legacy_01_introduction_2.tex <==
\section{Introduction}
\label{sec: intro}

Self-supervised learning has driven the rise of large foundation models, enabling training on vast, unlabeled data. This paradigm has proven effective in LLMs~\cite{radford2019language, brown2020language}, VLMs~\cite{caron2021emerging, bai2024sequential}, and video generation~\cite{peebles2023scalable, openai_sora_2024}. In contrast, 3D Vision still relies on ground-truth 3D geometry and camera poses labels~\cite{wang2024dust3r, hong2023lrm}, limiting its scalability and broader applications. Thus, we deviate the fully supervised learning paradigm and explore the scientific question: \textit{how far can we push a 3D Vision model without 3D supervision}?


In this paper, we present \textbf{\modelname{}}, a large multi-view 3D Vision model \textbf{trained with self-supervion}, exhibiting \textit{emerging 3D awareness}. Specifically, \modelname{} takes unposed and uncalibrated multi-view images or continuous video frames as input, it first recovers camera parameters, then \modelname{} reconstructs the scene representation and performs novel view rendering. \modelname{}'s training relies solely on photometric losses between input images and their renderings, requiring no 3D supervision and annotations.

To achieve successful self-supervised learning, we introduce \textbf{task-level} and \textbf{model-level} designs. From the perspective of the self-supervised learning task, it can be interpreted as 3D-aware \textit{images auto-encoding}~\cite{rumelhart1985learning, lai2021videoae}. From input images, \modelname{} first \textit{disentangles} them into camera parameters and scene representation, and then it \textit{re-entangles} the predicted representations back to images. To facilitate the efficacy for this disentanglement, we use \textbf{different information sources} to predict the representations and to provide supervision signal.
In detail, we split the input images into two sets. We use one set to predict the scene representation. We use the other set to provide photometric self-supervision, by using estimated poses of the second set to render the scene representation predicted from the first set. Thus, it avoids adopting trivial solutions that are not 3D-aware.

From the perspective of the model, \modelname{} is built with \textit{pure transformers} -- no 3D representation, rendering equation, and 3D-informed architectures. This design is motivated by self-supervised large models in other modalities~\cite{brown2020language, bai2024sequential, peebles2023scalable}, learning domain-specific knowledge with greater flexibility. The secret sauce to make this transformer-based model 3D-aware is \textbf{injecting the least ``3D'' prior} -- the \textit{ray structure}, as it simultaneously reveals the correlation between pixel (image), camera, and scene geometry. In detail, \modelname{} first predict camera poses, which are transformed into pixel-align Plücker ray maps~\cite{plucker1865xvii} to condition the following scene reconstruction. This representation turns out to be a strong prior for solving the chicken-and-egg structure and motion problem~\cite{cornell_sfm_lecture}. This is achieved, in our understanding, by letting camera and scene representations to \textit{regularize each other} to pursue the global minima in a smooth optimization landscape~\cite{zhang2024cameras}.



% our least ``3D'' prior is the bridging of scene, camera, and pixel using \textbf{rays}. The ray is a powerful physical concept, which simultaneously models the ray-pixel alignment relation in 2D space, and ray-scene geometry in 3D space. Specifically, \modelname{} first estimates camera parameters, including intrinsics and per-view camera poses. Then \modelname{} turns the predicted camera parameters as Plücker rays~\cite{} to condition scene reconstruction from the first image set. Finally, it uses these predicted rays of the second image set to query the scene representation and render target images. While jointly learning structure and motion is a classic \textit{chicken-and-egg problem}~\cite{}, the ray-based formulation turns out to be a strong prior. This is achieved, in our understanding, by letting camera and scene representations to \textbf{regularize each other} to pursue the global minima.


Conceptually, \modelname{} and video generation models can be two sides of a same coin -- video generation models are also built with transformers, with no 3D scene representation, learning from unlabeled videos, and showing emerging 3D awareness~\cite{openai_sora_2024}. However, we demonstrate that with our least ``3D'' prior of using the ray structure, we can achieve \textit{unsupervised control} of rendering viewpoint by disentangling the camera representation from the scene representation. We hope \modelname{} can inspire the following works building video generation models with unsupervised controls, without replying on supervised post-training~\cite{he2024cameractrl, kuang2025collaborative}. At the same time, we clarify that \modelname{} focuses on multi-view images of \textit{static scenes}. We believe extending our self-learning framework to dynamic videos is a possible way to scale up 3D Vision, enabling learning on any online video data. \modelname{} is the our first exploration towards this direction.


%\modelname{} supports different 3D representation, i.e., 3D Gaussians~\cite{} and latent set scene representation~\cite{}. When using the 3D Gaussian representation, \modelname{} benefits from the awareness of 3D geometry. When using the latent set scene representation, \modelname{} predicts a ``latent ray field'' as tokens, and uses transformer to model ray physics, i.e., how a ray propagate in space, reveals cross-view correlations, forms a scene representation and accumulates to a pixel. In this context, \modelname{} only has \textbf{the least ``3D'' priors}, which is using the ray structure to learn to predict light fields without 3D representations, architectures, and supervision.




We train \modelname{} on xxx


==> sections/legacy_04_method_0.tex <==
\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{figures/model.pdf}
    \vspace{-0.28in}
    \caption{\small{\textbf{\modelname{} Model framework.} 
    } \modelname{} takes in unposed and uncalibrated multi-view images and predicts per-view camera parameters and a scene representation, which supports novel view rendering. (\textbf{Left}) \modelname{} first estimate camera parameters, where one view is selected as the canonical reference view (in blue box). \modelname{} predicts the intrinsics and the relative camera poses of all views. The predicted cameras are then transformed into pixel-aligned Plücker ray maps. (\textbf{Middle}) \modelname{} use a subset of input images, $\mathcal{I}_\mathcal{A}$, as well as their previously predicted cameras, $\mathcal{R}_\mathcal{A}$, to output the scene representation, which can be either a latent set or 3D Gaussians. In this stage, the Plücker ray maps $\mathcal{R}_\mathcal{A}$ is an effective condition for scene reconstruction. (\textbf{Right}) \modelname{} can render a target image given the scene representation and a target camera. The rendering decoders and target camera parametrization are different for the two scene representations. During training, we use predicted cameras of $\mathcal{I}_\mathcal{B}$ for rendering $\hat{\mathcal{I}}_\mathcal{B}$, training \modelname{} end-to-end with self-supervised photometric losses.
    } 
    \label{fig: model}
    \vspace{-0.15in}
\end{figure*}


\section{\modelname{}}

In this section, we will first introduce the self-supervised task that \modelname{} performs (Sec.~\ref{sec: method_task}). Then, we present the \modelname{} model architecture (Sec.~\ref{sec: method_model}) to effectuate self-supervised learning. Finally, we introduce our designs to facilitate learning (Sec.~\ref{sec: method_learning}). 

\subsection{\modelname{} Self-supervised Task}
\label{sec: method_task}

We first formulate the input and outputs of \modelname{}, presenting the 3D Vision tasks that \modelname{} can perform. We then introduce the self-supervised learning task.

We focus on modeling static 3D scenes (no scene dynamics), which is a standard setting in multi-view 3D vision~\cite{}. Thus, we represent the scene with a scene representation and per-view camera parameters. The \textbf{input} of \modelname{} is a set of unposed and uncalibrated multi-view images $\mathcal{I}$. The \textbf{output} is the scene parametrization, i.e., camera intrinsics, per-view camera poses, and the scene representation, enabling 3D reconstruction and novel view synthesis. Importantly, the accurate prediction of these representation is achieved with fully \textbf{self-supervised learning}.

As discussed in Sec.~\ref{sec: intro}, denoting the input images set as $\mathcal{I}$, we split it into two \textit{non-overlapping} subsets $\mathcal{I}_\mathcal{A}$ and $\mathcal{I}_\mathcal{B}$, where $\mathcal{I}_\mathcal{A} \cup \mathcal{I}_\mathcal{B} = \mathcal{I}$ and  $\mathcal{I}_\mathcal{A} \cap \mathcal{I}_\mathcal{B} = \emptyset$. \modelname{} predict the \textit{scene representation from $\mathcal{I}_\mathcal{A}$}, and use predicted cameras that are correspond to images in \textit{$\mathcal{I}_\mathcal{B}$ for providing supervision} signal. Thus, \modelname{} renders images of $\hat{\mathcal{I}}_\mathcal{B}$ that corresponds to $\mathcal{I}_\mathcal{B}$, where we apply photometric losses
\begin{align}
    \mathcal{L} = \frac{1}{K_\mathcal{B}} \sum_{\hat{I} \in \hat{\mathcal{I}}_\mathcal{B}} (\texttt{MSE}(I, \hat{I}) + \lambda \cdot \texttt{Percep}(I, \hat{I})),
\end{align}
where $K_\mathcal{B} = \vert \mathcal{I}_\mathcal{B} \vert$ is the size (number of images) of $\mathcal{I}_\mathcal{B}$ , $I$ is the image of the input image set $\mathcal{I}_\mathcal{B}$ that corresponds to predicted $\hat{I}$, and $\lambda$ is the weight for perceptual loss~\cite{}.

In detail, the two sets are randomly sampled in training and are evenly sampled in an interleaved manner in testing.


% This self-supervised learning framework can be interpreted as information \textbf{auto-encoding with disentangled representations}~\cite{}. This perspective helps us understand the split of $\mathcal{I}_\mathcal{A}$ and $\mathcal{I}_\mathcal{B}$. \modelname{}'s encoder \textit{disentangles} the information of input images into the camera and scene representations, and its decoder \textit{re-entangles} them back as images. Without the data split, the model can cheat to minimize loss by adopting \textit{trivial solutions with no 3D-awareness}. Splitting inputs, which uses \textit{different information sources} to predict scene representation and provide supervision signal, is a \textbf{task-level regularization} to avoid trivial solutions.

% The second relates to self-supervised contrastive learning~\cite{}, which applies different augmentations to an image and assumes their high-level features are the same, leading to emerging semantic awareness. Naturally, the images in the two sets $\mathcal{I}_\mathcal{A}$ and $\mathcal{I}_\mathcal{B}$ can be seen as different ``augmentations'' of the same 3D scene under different camera poses. 


% Our \textbf{target} is learning a large  model, \modelname{}, in a \textit{self-supervised} manner to predict these representations. This means \modelname{} is able to do the \textbf{tasks}. During training, \modelname{} learns on a large amount of training samples to get generalizable priors. During testing, given a set of images, \modelname{} predicts these scene representations in a single feed-forward step.


% \modelname{}'s self-supervised learning can be understood as the \textit{3D-aware} \textbf{auto-encoding} of input images. From the image information, \modelname{} \textit{disentangles} two components, i.e., scene representation and per-view camera parameters. Then, \modelname{} \textit{re-entangles} the two components for decoding (rendering) the original input images. The loss is defined as their photometric discrepancy with the original inputs.

% To achieve meaningful disentanglement, one key of \modelname{} is \textbf{using different information sources} for predicting scene representation and providing supervision signal, avoiding model cheating with \textit{trivial solutions with no 3D-awareness}. Denoting the input images set as $\mathcal{I}$ and we split it into two \textit{non-overlapping} subsets $\mathcal{I}_\mathcal{A}$ and $\mathcal{I}_\mathcal{B}$, where $\mathcal{I}_\mathcal{A} \cup \mathcal{I}_\mathcal{B} = \mathcal{I}$ and  $\mathcal{I}_\mathcal{A} \cap \mathcal{I}_\mathcal{B} = \emptyset$. \modelname{} predict the scene representation from $\mathcal{I}_\mathcal{A}$, and use predicted cameras that are correspond to images in $\mathcal{I}_\mathcal{B}$ for providing supervision. Thus, \modelname{} decode images of $\hat{\mathcal{I}}_\mathcal{B}$, where we apply photometric losses
% \begin{align}
%     \mathcal{L} = \frac{1}{K_\mathcal{B}} \sum_{\hat{I} \in \hat{\mathcal{I}}_\mathcal{B}} (\texttt{MSE}(I, \hat{I}) + \lambda \cdot \texttt{Percep}(I, \hat{I})),
% \end{align}
% where $K_\mathcal{B}$ is the size of $\mathcal{I}_\mathcal{B}$ (number of images), $I$ is the image of the input image set $\mathcal{I}_\mathcal{B}$ that corresponds to predicted $\hat{I}$, and $\lambda$ is a weight for balancing the perceptual loss~\cite{}.


\subsection{\modelname{} Model}
\label{sec: method_model}

\noindent \textbf{Overview}. As introduced in Sec.~\ref{sec: method_task}, \modelname{} recovers camera parameters and scene representation from unposed and uncalibrated input images. A key design of \modelname{} model scheme is predicting the camera and scene representations in a \textbf{cascade} manner. This is motivated by our understanding that even noisy cameras can be a strong condition for better scene reconstruction, which is analogous to traditional methods and is in contrast with recent geometry-first large models~\cite{}. This design can provide mutual regularization of predicting pose and scene during training in our self-supervised learning framework. 



\modelname{} is a pure transformer-based model, which benefits from its scalability and flexibility.
As shown in Fig.~\ref{fig: model}, \modelname{} first tokenizes input images and uses a transformer-based camera encoder for predictingthe  camera parameters of all input views. In this step, the cameras are parameterized as intrinsics and $\texttt{SE(3)}$ poses. This parametrization benefits from its \textbf{low-dimensional} \textbf{geometric definiteness}, helping \textit{disentangle} image information from the camera representation.


\modelname{} then transforms the $\texttt{SE(3)}$ camera poses and intrinsics into Plücker rays~\cite{}, which is a pixel-aligned camera representation. They simultaneously model the ray-pixel alignment relation in 2D space and ray geometry in 3D space.
This representation benefits from its \textbf{fine-grained ray-level information} capturing the physical camera model, which serves as a better condition for reconstruction and benefits learning with its smoother optimization landscape~\cite{}.

From image and Plücker rays that correspond to the image set $\mathcal{I}_\mathcal{A}$, \modelname{} uses a transformer-based scene encoder to predict the scene representation, which can be either 3D Gaussians or the latent set scene representation.
Then \modelname{} uses the previously estimated cameras of $\mathcal{I}_\mathcal{B}$ for rendering $\hat{\mathcal{I}}_\mathcal{B}$, which provides supervision signal. Note that the two 3D representations have different rendering decoders. 
%3D Gaussians are rendered based on the alpha-blending ray marching. The latent set representation requires a learned decoder for rendering, introducing less 3D inductive bias to \modelname{} with using transformers to learn ray physics~\cite{}.


\vspace{0.02in}
\noindent \textbf{Image Tokenization}. For all $K$ input images $\mathcal{I} = \{ I_i \in \mathbb{R}^{H\times W\times 3} \vert i=1,...,K \}$, we patchify them into non-overlapping patches following ViT~\cite{}. Each patch is in $\mathbb{R}^{s\times s\times 3}$, where $s$ is the patch size. We use a linear layer to encode each patch into a token in $\mathbb{R}^d$, leading to a patch-aligned feature token map $f_i \in \mathbb{R}^{h\times w\times d}$ for each image, where $h=H/s$, $w=W/s$, and $d$ is the latent dimension.

We then add positional embeddings (p.e.) to the feature tokens, enabling the following model to be aware of the spatial location of the patch and which input image each token corresponds to. In detail, it includes the sinusoidal spatial p.e.~\cite{} and the sinusoidal image index p.e.~\cite{}, and we use a linear layer to fuse them. Specifically, the image index p.e. is shared across all tokens from the same image.
Finally, we reshape the token maps of all images as a set. Because the transformer is permutation invariant, we denote it as $\mathbf{f} \in \mathbb{R}^{Khw\times d}$. For the simplicity of notations, we will keep this notation style of latent token sets in the following contents.

\vspace{0.02in}
\noindent \textbf{Camera Encoder}. The camera encoder $\mathcal{E}_{cam}$ predicts camera parameters, i.e., camera pose and intrinsics, for all input images. We use a learnable pose token in $\mathbb{R}^{1\times d}$ as the initial feature for this prediction for all views. We repeat the token $K$ times and add them with image index p.e. to let them correspond to the $K$ images. We denote this camera feature initialization as $\mathbf{p} \in \mathbb{R}^{K\times d}$. We then use the camera encoder composed of full self-attention transformer layers to update the pose tokens, as 
\begin{align}
    \{\mathbf{f}^{*}, \mathbf{p}^{*}\} = \mathcal{E}_{cam}(\{\mathbf{f}, \mathbf{p} \}),
\end{align}
where $\{\cdot, \cdot \}$ denotes the joint set of two sets, $\mathbf{f}^{*}$ and $ \mathbf{p}^{*}$ are the updated tokens. We note that $\mathbf{f}^{*}$ is not used for the following computation; it is only used as context to update $\mathbf{f}$ in the transformer layers. For clarity, we formulate the transformer layers in the encoder as follows, which remains consistent throughout the rest of the paper:
\begin{align}
    \label{math: union_set}
    & \mathbf{y}^0 = \{\mathbf{f}, \mathbf{p} \}, \\
    & \mathbf{y}^{l} = \text{TransformerLayer}^l(\mathbf{y}^{l-1}), \tiny{l=1,...,l_T}\\
    & \{\mathbf{f}^*, \mathbf{p}^*\} = \text{split}(\mathbf{y}^{l_T}),
\end{align} 
where $l_T$ is the number of layers, and the $\text{split}$ operation recovers the two token sets (inversion to Eq.~\ref{math: union_set}).

Then we predict camera parameters for each image independently. For camera pose prediction, we follow prior works to predict relative camera poses, resolving pose ambiguity~\cite{}. We select one view as the canonical reference view and set its pose as a constant, e.g., identity rotation and zero translation. For each non-canonical view, we predict its relative camera pose regarding to the canonical view. Specifically, we parametrize the $\texttt{SO(3)}$ rotation matrix with 6D representation~\cite{}, leveraging its continuity. We formulate relative pose prediction using a two-layer MLP as follows:
\begin{align}
    p_i = \text{MLP}_{pose}([\mathbf{p}^{*}_c, \mathbf{p}^{*}_i]),
\end{align}
where $[\cdot, \cdot]$ denotes concatenation along the feature dimension, $\mathbf{p}^{*}_i$ and $\mathbf{p}^{*}_c$ (all in $ \mathbb{R}^{d}$) are the pose token for image $I_i$ and the canonical view. $p_i \in \mathbb{R}^{9}$ is predicted pose parameters. We then transform the predicted pose parameters to pose matrix, denoting the pose of image $I_i$ as $\mathbf{P}_i \in \texttt{SE(3)}$.

For intrinsics prediction, following prior works~\cite{}, we parametrize it with a focal length value, assuming i) the focal length for x-axis and y-axis of image are the same; ii) a constant intrinsics; and iii) the principal point is at the center of image. We predict focal length using a two-layer MLP:
\begin{align}
    \text{focal} = \text{MLP}_{focal}(\mathbf{p}^{*}_c).
\end{align}
Then we convert it to the intrinsics matrix $\mathbf{K} \in \mathbb{R}^{3\times 3}$.



\vspace{0.02in}
\noindent \textbf{Scene Encoder}. As discussed in Sec.~\ref{sec: method_learning}, we predict the scene representation from image set $\mathcal{I}_\mathcal{A}$ and additionally condition on its previously predicted camera parameters $\mathcal{P}_\mathcal{A} = \{(\mathbf{P}_i, \mathbf{K} ) | I_i \in \mathcal{I}_\mathcal{A}\}$.
We first transform $\mathcal{P}_\mathcal{A}$ to pixel-aligned Plücker rays~\cite{} for each image, denoted as $\mathcal{R} \in \mathbb{R}^{K\times H\times W \times 6}$. Similar to image inputs, we also tokenize the Plücker rays into patch-level feature tokens using a linear layer, denoted as $\mathbf{r} \in \mathbb{R}^{Khw\times d}$. We index the image and Plücker rays tokens to get the ones corresponds to the image set $\mathcal{I}_\mathcal{A}$, denoted as $\mathbf{f}_\mathcal{A}$ and $\mathbf{r}_\mathcal{A}$, which are both in $\mathbb{R}^{K_\mathcal{A}hw\times d}$. We use an MLP to fuse them along the feature dimension: 
\begin{align}
    \mathbf{x}_\mathcal{A} = \text{MLP}_{fuse}([\mathbf{f}_\mathcal{A}, \mathbf{r}_\mathcal{A}]),
\end{align}
where $\mathbf{x}_\mathcal{A} \in \mathbb{R}^{K_\mathcal{A}hw\times d}$ denotes the tokens after this information fusion.
Importantly, we use $\mathbf{f}$ rather than $\mathbf{f}^*$ for this fusion. This avoids the leakage of image information of set $\mathcal{I}_\mathcal{B}$, as transformers in the camera encoder, which produces $\mathbf{f}^*$, has a global context and can also see $\mathcal{I}_\mathcal{B}$ information.

We then use a scene encoder $\mathcal{E}_{scene}$ with full self-attention transformer layers to predict the scene representation. As discussed previously, \modelname{} supports different scene representations, i.e., 3D Gaussians and latent sets. We here first introduce the encoder for predicting the latent set representation. For initializing this scene representation, we use a set of learnable tokens, denoted as $\mathbf{z}_{\text{latent}} \in \mathbb{R}^{L}\times d$, where $L$ is the size (number of tokens) of the latent set representation. We formulate it as:
\begin{align}
    \{ \mathbf{z}^*_{\text{latent}},  \mathbf{x}^*_\mathcal{A} \} = \mathcal{E}_{scene}(\{ \mathbf{z}_{\text{latent}},  \mathbf{x}_\mathcal{A} \}).
\end{align}
The update rule is the same as the transformer layers in the camera encoder $\mathcal{E}_{cam}$. Here $\mathbf{z}^*_{\text{latent}}$ is the final latent set scene representation, which is trained to be a 3D-aware compression of inputs $\mathcal{I}_\mathcal{A}$.  And $\mathbf{x}_\mathcal{A}^{*}$ is discarded.

Differently, when using the 3D Gaussian representation, \modelname{} predicts pixel-aligned 3D Gaussians. The scene encoder only updates the input tokens, as:
\begin{align}
     \mathbf{x}_\mathcal{A}^* = \mathcal{E}_{scene}(\mathbf{x}_\mathcal{A}).
\end{align}
We decode 3D Gaussians at the patch level using an MLP:
\begin{align}
    \mathbf{Z}_{\text{gs}} = \text{MLP}_{gs}(\mathbf{x}_\mathcal{A}^*),
\end{align}
where $\mathbf{Z} \in \mathbb{R}^{K_\mathcal{A}hw\times (s^2 d_{gs})}$ is the patch-aligned decoded Gaussian attributes, and then we reshape is to pixel-aligned Gaussians in $\mathbb{R}^{K_\mathcal{A}HW\times (d_{gs})}$, where $H=h\cdot s$ and $W=w\cdot s$.


% $\mathbf{z}^{*}_j$ is the $j^{th}$ token of $\mathbf{z}^{*}$, $\mathbf{Z}_j \in \mathbb{R}^{s^2\cdot d_{gs}}$ represents the decoded Gaussians, where $d_{gs}$ is the dimension of Gaussian attributes. We then reshape $\mathbf{Z}_j$ to $\mathbb{R}^{s^2 \times d_{gs}}$, representing the $s^2$ predicted Gaussian from this token. We denote all predicted Gaussians as $\mathbf{Z} \in \mathbb{R}^{K_\mathcal{A}HW\times d_{gs}}$.

\vspace{0.02in}
\noindent \textbf{Rendering Decoder}. We first formulate the rendering decoder, and then introduce how it is used. When using the latent set representation, we use a transformer-based decoder for rendering, following LVSM~\cite{}.

Generally, for a target image to render, we first represent it as pixel-aligned Plücker rays, we first tokenize it using a linear layer, denoting the target tokens to be updated as $\mathbf{r} \in \mathbb{R}^{hw \times d}$. Then we update them by fusing scene information, using a decoder with full self-attention transformer layers:
\begin{align}
    \{ \mathbf{r}^{*}, \mathbf{z}'_\text{latent} \} = \mathcal{D}_{render}(\{ \mathbf{r}, \mathbf{z}^{*}_\text{latent} \}),
\end{align}
where $\mathbf{z}'$ is later discarded. Then, we use an MLP to decode the RGB values at the patch level as:
\begin{align}
    \hat{I} = \text{MLP}_{rgb}(\mathbf{r}^{*}),
\end{align}
where $\hat{I} \in \mathbb{R}^{hw\times (3s^2)}$, and then we recover its 2D spatial structure by reshaping it to $\mathbb{R}^{H\times W\times 3}$.

When using the 3D Gaussian representation $\mathbf{Z}_{\text{gs}}$, we render the target images given a target camera $(\mathbf{P}, \mathbf{K})$, based on its rendering equation~\cite{}.



During training, we render the images of $\hat{\mathcal{I}}_B = \{ \hat{I} | I \in \mathcal{I}_\mathcal{B}\}$ for providing self-supervision, as discussed in Sec.~\ref{sec: method_task}. We use the camera parameters predicted by the camera encoder, as $\mathcal{P}_\mathcal{B} = (\mathbf{P}_i, \mathbf{K} ) | I_i \in \mathcal{I}_\mathcal{B}\}$, and its converted Plücker ray maps $\mathcal{R}_\mathcal{B}$, to render $\hat{\mathcal{I}}_B$ for the scene representations of 3D Gaussians and the latent set, respectively.



\subsection{Designs for Facilitating \modelname{} Learning}
\label{sec: method_learning}
\modelname{} works on multi-view image inputs, which can be either continuous video frames or an unordered image set.
In this section, we present two designs to improve the self-learning efficacy for video frame input.


\noindent \textbf{Canonical view selection}. Prior works~\cite{} usually select the first image in the video frame sequence as the canonical view. In contrast, we select the frame at the middle time-step as canonical when using continuous video frame inputs. In this context, the pose prediction $\text{MLP}_{pose}$ initialized with a zero mean for its weights will have a small data variance. Otherwise, when using the first frame as canonical, the variance is much larger. We find this design helps the self-supervised learning of pose prediction.

\noindent \textbf{Curriculum}. We gradually increase the training difficulty by sampling video frames with an increasing distance range. With a proper model initialization of camera pose estimation, it first learns from images with small camera baselines (by predicting nearly constant poses), benefiting the following training with larger camera baselines.

% \noindent \textbf{Initialization of camera parameter prediction}. 

